Exploiting temporal consistency for real-time video depth estimation

Accuracy of depth estimation from static images has been significantly improved recently, by exploiting hierarchical features from deep convolutional neural networks (CNNs). Compared with static images, vast information exists among video frames and can be exploited to improve the depth estimation performance. In this work, we focus on exploring temporal information from monocular videos for depth estimation. Specifically, we take the advantage of convolutional long short-term memory (CLSTM) and propose a novel spatial-temporal CSLTM (ST-CLSTM) structure. Our ST-CLSTM structure can capture not only the spatial features but also the temporal correlations/consistency among consecutive video frames with negligible increase in computational cost. Additionally, in order to maintain the temporal consistency among the estimated depth frames, we apply the generative adversarial learning scheme and design a temporal consistency loss. The temporal consistency loss is combined with the spatial loss to update the model in an end-to-end fashion. By taking advantage of the temporal information, we build a video depth estimation framework that runs in real-time and generates visually pleasant results. Moreover, our approach is flexible and can be generalized to most existing depth estimation frameworks. Code is available at: https://tinyurl.com/STCLSTM

==> main.bib.1 <==
\usepackage{stringstrings}
@STRING{ACCV  = {Proc. Asian Conf. Comp. Vis.}}
@STRING{CVPR  = {Proc. IEEE Conf. Comp. Vis. Patt. Recogn.}}
@STRING{ECCV  = {Proc. Eur. Conf. Comp. Vis.}}
@STRING{BMVC  = {Proc. British Machine  Vis. Conf.}}
@STRING{ICCV  = {Proc. IEEE Int. Conf. Comp. Vis.}}
@STRING{ICIP  = {Proc. IEEE Int. Conf. Image Process.}}
@STRING{ICPR  = {Proc. Int. Conf. Patt. Recogn.}}

@STRING{ICML  = {Proc. Int. Conf. Mach. Learn.}}
@STRING{ICLR  = {Proc. Int. Conf. Learn. Representations}}
@STRING{UAI   = {Proc. Conf. Uncertainty in Artificial Intelli.}}
@STRING{COLT  = {Proc. Annual Conf. Learn. Theory}}


@STRING{IJCAI   = {Proc. Int. Joint Conf. Artificial Intell.}}
@STRING{AAAI    = {Proc. {AAAI} Conf. Artificial Intell.}}


@STRING{AISTATS = {Proc. Int. Conf. Artificial Intell. \& Stat.}}
@STRING{NIPS    = {Proc. Advances in Neural Inf. Process. Syst.}}
@STRING{NeurIPS    = {Proc. Advances in Neural Inf. Process. Syst.}}
@STRING{KDD     = {Proc. {ACM SIGKDD} Int. Conf. Knowledge discovery \& data mining}}
@STRING{PAKDD     = {Proc. Pacific-Asia. Conf. Knowledge discovery \& data mining}}

@STRING{MM      = {Proc. {ACM} Int. Conf. Multimedia}}
@STRING{ACMMM   = {Proc. {ACM} Int. Conf. Multimedia}}

@STRING{IROS   = {Proc. {IEEE/RSJ} Int. Conf. Intelligent Robots \& Systems}}
@STRING{AVSS   = {Proc. IEEE Int. Conf. Advanced Video Signal-based Surveillance}}
@STRING{PETS   = {Proc. IEEE Int. Workshop on Performance Evaluation for Tracking and Surveillance}}
@STRING{TOMM   = {ACM Trans. Multimedia Computing, Communications, and Applications}}

@STRING{JMLR    = {J. Mach. Learn. Res.}}
@STRING{ML      = {Mach. Learn.}}
@STRING{MS      = {Management Sci.}}

@STRING{PR      = {Pattern Recogn.}}

@STRING{TAC         = "{IEEE} Trans. Autom. Control"}
@STRING{TCSVT       = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{TSP         = "{IEEE} Trans. Signal Process."}
@STRING{TSTSP       = "{IEEE} J. Sel. Topics Signal Process."}


@STRING{TIT         = "{IEEE} Trans. Inf. Theory"}
@STRING{TKDE        = "{IEEE} Trans. Knowl. Data Eng."}

@STRING{TNN         = "{IEEE} Trans. Neural Netw."}
@STRING{TNNLS       = "{IEEE} Trans. Neural Netw. \& Learn. Syst."}
@STRING{TIP         = "{IEEE} Trans. Image Process."}
@STRING{TMM         = "{IEEE} Trans. Multimedia"}


@STRING{JRA         = "{IEEE} J. Robot. Autom."}
@STRING{TPAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}

@STRING{TRA         = "{IEEE} Trans. Robot. Autom."}
@STRING{TRO         = "{IEEE} Trans. Robot."}
@STRING{TSMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{TSMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{TSMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{TSMCC       = "{IEEE} Trans. Syst. Man, Cybern. {C}"}

@STRING{IEEE_PROC   = "Proc. {IEEE}"}
@STRING{IEEEPROC    = "Proc. {IEEE}"}

@STRING{IJCV  = "Int. J. Comput. Vision"}
@STRING{CVIU  = {Comp. Vis. Image Understanding}}

@STRING{CoRR  = {arXiv: Comp. Res. Repository}}

% added by hkzhang

@STRING{ DV  = {Int. Conf.  3D Vision}}
@STRING{ICRA  = {Proc. IEEE Int. Conf. Robotics Automation.}}
@STRING{WACV  = {IEEE Winter. Conf.  App. Comp. Vis.}}
@STRING{ICASSP  = {Proc. IEEE Int. Conf. Acoust. Speech Signal Process.}}
@STRING{TMI         = "{IEEE} Trans. Med. Imaging"}



@inproceedings{paisitkriangkrai2015learning,
  title={Learning to rank in person re-identification with metric ensembles},
  author={Paisitkriangkrai, Sakrapee and Shen, Chunhua and Van Den Hengel, Anton},
  booktitle=CVPR,
  pages={1846--1855},
  year={2015}
}

@inproceedings{market1501,
  title={Scalable person re-identification: A benchmark},
  author={Zheng, Liang and Shen, Liyue and Tian, Lu and Wang, Shengjin and Wang, Jingdong and Tian, Qi},
  booktitle=ICCV,
  pages={1116--1124},
  year={2015}
}
@inproceedings{duke,
  title={Unlabeled samples generated by gan improve the person re-identification baseline in vitro},
  author={Zheng, Zhedong and Zheng, Liang and Yang, Yi},
  booktitle=ICCV,
  pages={3754--3762},
  year={2017}
}


@misc{Authors14,
 author = {Authors},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture  submission ID 324. Supplied as additional material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {Authors},
 title = {Frobnication tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {A. Alpher},
title = {Frobnication},
journal = {Journal of Foo},
volume = 12, 
number = 1, 
pages = {234--778}, 
year = 2002
}

@article{Alpher03,
author = {A. Alpher and  J.~P.~N. Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13, 
number = 1, 
pages = {234--778}, 
year = 2003
}

@article{Alpher04,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe and G. Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14, 
number = 1, 
pages = {234--778}, 
year = 2004
}

%%============%%

@article{zhou2018unsupervised,
  title={Unsupervised Learning of Monocular Depth Estimation with Bundle Adjustment, Super-Resolution and Clip Loss},
  author={Zhou, Lipu and Ye, Jiamin and Abello, Montiel and Wang, Shengze and Kaess, Michael},
  journal=CoRR,
  volume={abs/1812.03368},
  year={2018}
}

@inproceedings{fu2018deep,
  title={Deep ordinal regression network for monocular depth estimation},
  author={Fu, Huan and Gong, Mingming and Wang, Chaohui and Batmanghelich, Kayhan and Tao, Dacheng},
  booktitle=CVPR,
  pages={2002--2011},
  year={2018}
}


@inproceedings{mahjourian2018unsupervised,
  title={Unsupervised learning of depth and ego-motion from monocular video using 3d geometric constraints},
  author={Mahjourian, Reza and Wicke, Martin and Angelova, Anelia},
  booktitle=CVPR,
  pages={5667--5675},
  year={2018}
}

@inproceedings{eigen2014depth,
  title={Depth map prediction from a single image using a multi-scale deep network},
  author={Eigen, David and Puhrsch, Christian and Fergus, Rob},
  booktitle=NIPS,
  pages={2366--2374},
  year={2014}
}

@inproceedings{hu2019revisiting,
  title={Revisiting single image depth estimation: toward higher resolution maps with accurate object boundaries},
  author={Hu, Junjie and Ozay, Mete and Zhang, Yan and Okatani, Takayuki},
  booktitle=WACV,
  pages={1043--1051},
  year={2019},
  organization={IEEE}
}

@inproceedings{laina2016deeper,
  title={Deeper depth prediction with fully convolutional residual networks},
  author={Laina, Iro and Rupprecht, Christian and Belagiannis, Vasileios and Tombari, Federico and Navab, Nassir},
  booktitle={International conference on 3D vision},
  pages={239--248},
  year={2016},
  organization={IEEE}
}

@inproceedings{mikolov2011extensions,
  title={Extensions of recurrent neural network language model},
  author={Mikolov, Tom{\'a}{\v{s}} and Kombrink, Stefan and Burget, Luk{\'a}{\v{s}} and {\v{C}}ernock{\`y}, Jan and Khudanpur, Sanjeev},
  booktitle=ICASSP,
  pages={5528--5531},
  year={2011},
  organization={IEEE}
}

@inproceedings{graves2013speech,
  title={Speech recognition with deep recurrent neural networks},
  author={Graves, Alex and Mohamed, Abdel-rahman and Hinton, Geoffrey},
  booktitle=ICASSP,
  pages={6645--6649},
  year={2013},
  organization={IEEE}
}

@article{ballas2015delving,
  title={Delving deeper into convolutional networks for learning video representations},
  author={Ballas, Nicolas and Yao, Li and Pal, Chris and Courville, Aaron},
  journal=CoRR,
  volume={abs/1511.06432},
  year={2015}
}

@inproceedings{song2018pyramid,
  title={Pyramid dilated deeper convlstm for video salient object detection},
  author={Song, Hongmei and Wang, Wenguan and Zhao, Sanyuan and Shen, Jianbing and Lam, Kin-Man},
  booktitle=ECCV,
  pages={715--731},
  year={2018}
}

@article{jiang2017predicting,
  title={Predicting video saliency with object-to-motion CNN and two-layer convolutional LSTM},
  author={Jiang, Lai and Xu, Mai and Wang, Zulin},
  journal=CoRR,
  volume={abs/1709.06316},
  year={2017}
}

@inproceedings{liu2016spatio,
  title={Spatio-temporal LSTM with trust gates for 3D human action recognition},
  author={Liu, Jun and Shahroudy, Amir and Xu, Dong and Wang, Gang},
  booktitle=ECCV,
  pages={816--833},
  year={2016},
  organization={Springer}
}

@article{mirowski2016learning,
  title={Learning to navigate in complex environments},
  author={Mirowski, Piotr and Pascanu, Razvan and Viola, Fabio and Soyer, Hubert and Ballard, Andrew J and Banino, Andrea and Denil, Misha and Goroshin, Ross and Sifre, Laurent and Kavukcuoglu, Koray and others},
  journal=CoRR,
  volume={abs/1611.03673},
  year={2016}
}

@inproceedings{borghi2017poseidon,
  title={Poseidon: Face-from-depth for driver pose estimation},
  author={Borghi, Guido and Venturelli, Marco and Vezzani, Roberto and Cucchiara, Rita},
  booktitle=CVPR,
  pages={4661--4670},
  year={2017}
}

@inproceedings{xie2016deep3d,
  title={Deep3d: Fully automatic 2d-to-3d video conversion with deep convolutional neural networks},
  author={Xie, Junyuan and Girshick, Ross and Farhadi, Ali},
  booktitle=ECCV,
  pages={842--857},
  year={2016},
  organization={Springer}
}

@article{liu2016learning,
  title={Learning depth from single monocular images using deep convolutional neural fields},
  author={Liu, Fayao and Shen, Chunhua and Lin, Guosheng and Reid, Ian},
  journal=TPAMI,
  volume={38},
  number={10},
  pages={2024--2039},
  year={2016},
  publisher={IEEE}
}

@inproceedings{wang2015towards,
  title={Towards unified depth and semantic prediction from a single image},
  author={Wang, Peng and Shen, Xiaohui and Lin, Zhe and Cohen, Scott and Price, Brian and Yuille, Alan L},
  booktitle=CVPR,
  pages={2800--2809},
  year={2015}
}

@inproceedings{xingjian2015convolutional,
  title={Convolutional LSTM network: A machine learning approach for precipitation nowcasting},
  author={Xingjian, Shi and Chen, Zhourong and Wang, Hao and Yeung, Dit-Yan and Wong, Wai-Kin and Woo, Wang-chun},
  booktitle=NIPS,
  pages={802--810},
  year={2015}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle=NIPS,
  pages={2672--2680},
  year={2014}
}

@inproceedings{isola2017image,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  booktitle=CVPR,
  pages={1125--1134},
  year={2017}
}

@article{mahmood2018unsupervised,
  title={Unsupervised reverse domain adaptation for synthetic medical images via adversarial training},
  author={Mahmood, Faisal and Chen, Richard and Durr, Nicholas J},
  journal=TMI,
  volume={37},
  number={12},
  pages={2572--2581},
  year={2018},
  publisher={IEEE}
}

@inproceedings{almalioglu2018ganvo,
  title={{GANVO}: Unsupervised Deep Monocular Visual Odometry and Depth Estimation with Generative Adversarial Networks},
  author={Almalioglu, Yasin and Saputra, Muhamad Risqi  and de Gusmao, Pedro  and Markham, Andrew and Trigoni, Niki},
  booktitle=ICRA,
  year={2019}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal=CoRR,
  volume={abs/1409.1556},
  year={2014}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle=CVPR,
  pages={770--778},
  year={2016}
}

@inproceedings{hu2018squeeze,
  title={Squeeze-and-excitation networks},
  author={Hu, Jie and Shen, Li and Sun, Gang},
  booktitle=CVPR,
  pages={7132--7141},
  year={2018}
}

@inproceedings{chen2018encoder,
  title={Encoder-decoder with atrous separable convolution for semantic image segmentation},
  author={Chen, Liang-Chieh and Zhu, Yukun and Papandreou, George and Schroff, Florian and Adam, Hartwig},
  booktitle=ECCV,
  pages={801--818},
  year={2018}
}

@inproceedings{long2015fully,
  title={Fully convolutional networks for semantic segmentation},
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle=CVPR,
  pages={3431--3440},
  year={2015}
}

@article{karsch2014depth,
  title={Depth transfer: Depth extraction from video using non-parametric sampling},
  author={Karsch, Kevin and Liu, Ce and Kang, Sing Bing},
  journal=TPAMI,
  volume={36},
  number={11},
  pages={2144--2158},
  year={2014},
  publisher={IEEE}
}

@article{saxena2009make3d,
  title={Make3d: Learning 3d scene structure from a single still image},
  author={Saxena, Ashutosh and Sun, Min and Ng, Andrew Y},
  journal=TPAMI,
  volume={31},
  number={5},
  pages={824--840},
  year={2009},
  publisher={IEEE}
}

@inproceedings{liu2014discrete,
  title={Discrete-continuous depth estimation from a single image},
  author={Liu, Miaomiao and Salzmann, Mathieu and He, Xuming},
  booktitle=CVPR,
  pages={716--723},
  year={2014}
}

@inproceedings{li2015depth,
  title={Depth and surface normal estimation from monocular images using regression on deep features and hierarchical crfs},
  author={Li, Bo and Shen, Chunhua and Dai, Yuchao and Van Den Hengel, Anton and He, Mingyi},
  booktitle=CVPR,
  pages={1119--1127},
  year={2015}
}

@inproceedings{liu2015deep,
  title={Deep convolutional neural fields for depth estimation from a single image},
  author={Liu, Fayao and Shen, Chunhua and Lin, Guosheng},
  booktitle=CVPR,
  pages={5162--5170},
  year={2015}
}


@inproceedings{eigen2015predicting,
  title={Predicting depth, surface normals and semantic labels with a common multi-scale convolutional architecture},
  author={Eigen, David and Fergus, Rob},
  booktitle=ICCV,
  pages={2650--2658},
  year={2015}
}

@inproceedings{chakrabarti2016depth,
  title={Depth from a single image by harmonizing overcomplete local network predictions},
  author={Chakrabarti, Ayan and Shao, Jingyu and Shakhnarovich, Greg},
  booktitle=NIPS,
  pages={2658--2666},
  year={2016}
}

@inproceedings{li2017two,
  title={A two-streamed network for estimating fine-scaled depth maps from single {RGB} images},
  author={Li, Jun and Klein, Reinhard and Yao, Angela},
  booktitle=ICCV,
  pages={3372--3380},
  year={2017}
}

@inproceedings{mal2018sparse,
  title={Sparse-to-dense: Depth prediction from sparse depth samples and a single image},
  author={Mal, Fangchang and Karaman, Sertac},
  booktitle=ICRA,
  pages={1--8},
  year={2018},
  organization={IEEE}
}

@inproceedings{xu2018pad,
  title={Pad-net: multi-tasks guided prediction-and-distillation network for simultaneous depth estimation and scene parsing},
  author={Xu, Dan and Ouyang, Wanli and Wang, Xiaogang and Sebe, Nicu},
  booktitle=CVPR,
  pages={675--684},
  year={2018}
}

@inproceedings{godard2017unsupervised,
  title={Unsupervised monocular depth estimation with left-right consistency},
  author={Godard, Cl{\'e}ment and Mac Aodha, Oisin and Brostow, Gabriel },
  booktitle=CVPR,
  pages={270--279},
  year={2017}
}

@inproceedings{kuznietsov2017semi,
  title={Semi-supervised deep learning for monocular depth map prediction},
  author={Kuznietsov, Yevhen and Stuckler, Jorg and Leibe, Bastian},
  booktitle=CVPR,
  pages={6647--6655},
  year={2017}
}

@inproceedings{JHLee2018,
  title={Single-Image Depth Estimation Based on Fourier Domain Analysis},
  author={Jae-Han Lee and Minhyeok Heo and Kyung-Rae Kim and Chang-Su Kim},
  booktitle=CVPR,
  year={2018}
}

@inproceedings{mayer2016large,
  title={A large dataset to train convolutional networks for disparity, optical flow, and scene flow estimation},
  author={Mayer, Nikolaus and Ilg, Eddy and Hausser, Philip and Fischer, Philipp and Cremers, Daniel and Dosovitskiy, Alexey and Brox, Thomas},
  booktitle=CVPR,
  pages={4040--4048},
  year={2016}
}

@article{paszke2017automatic,
  title={Automatic differentiation in pytorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  url={https://pytorch.org/},
  year={2017}
}

@article{cao2016estimating,
  title={Estimating Depth from Monocular Images as Classification Using Deep Fully Convolutional Residual Networks},
  author={Cao, Yuanzhouhan and Wu, Zifeng and Shen, Chunhua},
  journal=TCSVT,
  volume={28},
  issue={11},
  pages={3174--3182},
  year={2018},
  publisher={IEEE}
}

@inproceedings{zach2007duality,
  title={A duality based approach for realtime TV-L 1 optical flow},
  author={Zach, Christopher and Pock, Thomas and Bischof, Horst},
  booktitle={Proc. Annual Symp. German Assoc. Pattern Recogn.},
  pages={214--223},
  year={2007},
  organization={Springer}
}

@article{wang2004image,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan  and Sheikh, Hamid  and Simoncelli, Eero},
  journal=TIP,
  volume={13},
  number={4},
  pages={600--612},
  year={2004}
}

@inproceedings{Yin2019enforcing,
  title={Enforcing geometric constraints of virtual normal for depth prediction},
  author={Yin, Wei and Liu, Yifan and Shen, Chunhua and Yan, Youliang},
  booktitle=ICCV,
  year={2019}
}

@article{Rethinking18GAN,
  title={Rethinking Monocular Depth Estimation with Adversarial Training},
  author={
  Richard Chen	and
Faisal Mahmood	and	
Alan Yuille	and	
Nicholas J. Durr},
  journal=CoRR,
  year={2018}
}


@inproceedings{PoseNet,
  title={Adversarial {PoseNet}: A Structure-aware Convolutional Network for Human Pose Estimation},
  author={Yu Chen and
  Chunhua Shen and Xiu-Shen Wei  and Lingqiao Liu and Jian Yang},
  booktitle=ICCV,
  year={2017}
}




